Don't Let Me Down! Offloading Robot VFs Up to the Cloud

Recent trends in robotic services propose offloading robot functionalities to the Edge to meet the strict latency requirements of networked robotics. However, the Edge is typically an expensive resource and sometimes the Cloud is also an option, thus, decreasing the cost. Following this idea, we propose Don't Let Me Down! (DLMD), an algorithm that promotes offloading robot functions to the Cloud when possible to minimize the consumption of Edge resources. Additionally, DLMD takes the appropriate migration, traffic steering, and radio handover decisions to meet robotic service requirements as strict latency constraints. In the paper, we formulate the optimization problem that DLMD aims to solve, compare DLMD performance against state of art, and perform stress tests to assess DLMD performance in small & large networks. Results show that DLMD (i) always finds solutions in less than 30ms; (ii) is optimal in a local warehousing use case, and (iii) consumes only 5% of the Edge resources upon network stress.

==> AAN.tex <==
\begin{tikzpicture}[font=\scriptsize,
  radiounit/.style={rectangle,draw,fill=white!20},
  server/.style={rectangle,draw,fill=white!20},
  vf/.style={draw=black,fill=white!20,circle, inner sep=2.5pt,font=\tiny},
  line/.style={dotted, black!60,->,
    edge from parent path={(\tikzparentnode.south) |- (\tikzchildnode.west)}},
 % first/.style={level distance=6ex},
  %second/.style={level distance=12ex},
  %third/.style={level distance=18ex},
  %level 1/.style={sibling distance=5em}
  % Define arrow style
   % connectedline/.style={ ->,thick,shorten <=2pt, shorten >=2pt,},
    %graphs/every graph/.style={edges=rounded corners},
    skip loop/.style={to path={-- ++(0,#1) -| (\tikztotarget)}}
  ]
  \pgfmathsetmacro{\below}{-1.4}
        \pgfmathsetmacro{\aboveAbove}{1.7}
        \pgfmathsetmacro{\aboveBelow}{1}
        \pgfmathsetmacro{\middle}{-.47}
        \pgfmathsetmacro{\middleAbove}{-.17}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %%% Hardware %%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \coordinate
      child[grow=left] {node[server,anchor=east,align=center](c){Cloud}}
      child[grow=right]{node[server,anchor=west,align=center](fe){Far Edge}}
     % \drawAlong{(right)}{\Radius}{\Separation}{120}{60}
      child[grow=down,level distance=0ex]{node (fork){}}
   [edge from parent fork down]
    child{node[radiounit](s) {Switch}
    child{node[radiounit](p3) {PoA\textsubscript{3}}}
    child{node[radiounit](p2) {PoA\textsubscript{2}}}
    child{node[radiounit](p1) {PoA\textsubscript{1}}}
    child{node[radiounit](p4) {PoA\textsubscript{4}}}
    child{node[radiounit] (p5){PoA\textsubscript{5}}}
    child{node[radiounit](p6) {PoA\textsubscript{6}}}};
    \node[radiounit,align=center] (r) at ($(p1)-(0,1)$) {robot};
   \node[circle,fill=white,inner sep=0,font=\tiny] at (p1.south east) {$R_1$};
   \node[circle,fill=white,inner sep=0,font=\tiny] at (r.south east) {$r_1$};
   \node[circle,fill=white,inner sep=0,font=\tiny] (p6annot) at (p6.south east) {$R_6$};
   %\draw[dashed,very thick,draw=black]($(r.north)+ (2mm,0)$) -| ($(p1)+(1mm,0)$);
   %\draw[->,dashed,very thick,draw=black]
  % ($(p1)+(1mm,0)- (2mm,0) $) -- (s);
   %\draw[->,dashed,very thick,draw=black](s) -- (ne);
   %\draw[->,dashed,very thick,draw=black](s) -- (c);
   %\draw[vf](3.4,1.1) circle(1cm);
  \node(ne)[server,align=center] at (2.1,\below-.1){Near Edge};
   \node[circle,fill=white,inner sep=0,font=\tiny] at (ne.south east) {$n_1$};
   \draw[draw=black](s) -- (ne); 
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%% Virtual functions Placement %%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \node(rd)[vf,align=center] at ($(ne)+(1.8,0)$) {Remote\\driving};
   \node (rdTop) at ($(rd.north west)+(0,.2)$) {};
   \draw[->,dashed] (rd.north west) -- (rdTop) -- node[midway,above]{$P(v_1,n_1)=1$} (ne.north |- rdTop) -- (ne.north);

   \node[circle,fill=white!20,inner sep=0,font=\tiny] at (rd.south east) {$v_2$};
   %\node(mc)[vf,align=center] at ($(c)-(1.5,0)$) {Metrics\\collection};
   %\draw[->,dashed] (mc) -- ($(c.west)-(.1,0)$);
  % \node[circle,fill=white!20,inner sep=0,font=\tiny] at (mc.south east) {$v_3$};
   \node(ro) [vf,align=center] at ($(r)-(1.45,0)$) {Robot\\drivers};
   \node[circle,fill=white!20,inner sep=0,font=\tiny] at (ro.south east) {$v_1$};
   \draw[->,dashed] (ro) -- ($(r.west)-(.1,0)$);
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %%%  Notations  %%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % \node[fill=white,draw=gray, align=left] at (-1,\middleAbove-.3){$P(\cdot)$};
    % \node[fill=white,draw=gray, align=left] at (-2.1,\below-.3){$\sigma(\cdot)$,$d(\cdot)$,$\lambda(\cdot)$};
    %\node[fill=white,draw=gray, align=left] at (2.1,\below-.3){$\sigma(\cdot)$,$d(\cdot)$,$\lambda(\cdot)$};
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %%%  path  %%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \draw[dashed,very thick] (r) --  node[pos=0.3,right] {$\phi(r_1,R_1)=1$} (p1);
    \path(p1) edge[very thick, skip loop=7mm](s);
    \path(s) edge[very thick](ne);
    \path(s) edge[] node[pos=.3,anchor=east]{$d(w_1,n_3)=27$ms} ($(fork)+(0,.02)$);
    %\path($(fork)+(.02,0)$) edge[very thick](c);



    %% Internet cloud
    \node[cloud, fill=white, draw=black,align=center,font=\tiny,minimum width = 0.001cm,minimum height = 0.01cm,  cloud ignores aspect] (aan) at ($(c)+(1.2,0)$) {Internet};


    %% Math labels
    \node[font=\tiny,fill=white,inner sep=0] at (c.south east) {$n_3$};
    \node[font=\tiny,fill=white,inner sep=0] at (fe.south east) {$n_2$};
    \node[font=\tiny,fill=white,inner sep=0] at (s.south east) {$w_1$};
    \node[fill=white,anchor=north,align=center] at ($(p6)-(0,.35)$) {$\sigma_{R_6}(r_1)=$-87dB };

    %%%%%%%%%%%%%%%% AAN %%%%%%%%%%%%%%%%%%%%
    %\path[dotted,very thick] ($(aan) + (.77,0)$) edge[bend right=80]  node[right] {} (c);
    %\path[dotted,very thick] ($(aan) - (.75,0)$) edge[bend left=30]  node[right] {} (p1);
\end{tikzpicture}


==> system.tex <==
\section{COTORRA architecture}
\label{sec:system}
{\color{red}{In progress}}COTORRA has three layers as following:
\begin{itemize}
\item Plug-in layer
\item Core layer
\subitem \textbf {Middle-ware} 
\subitem \textbf {Measurements}
\subitem \textbf {Network Control}
\end{itemize}
It is worth mentioning that the architecture is designed to be compliant
with Multi-access Edge Computing (MEC)~\cite{etsi.mec}.
In particular, it is possible to implement the Plug-ins and
Core layer building blocks as a set of autonomous applications and context-aware services running on top of a standard MEC virtualization infrastructure. This implies that    COTORRA contributes to the experimental evaluation of MEC compliant applications.

\begin{comment}

\subsection{COTORRA Core layer}
\label{subsec:cotorra_core}
COTORRA Core layer is a set of
building blocks, namely, the Robot Middleware,
Network Control, and Measurements
building block. Every building block has an API
to interact with the testbed, and report
data to the Plug-ins layer.
The following details the functionality of
each building block:

\begin{itemize}
    \item \textbf{Robot Middleware} building block
     collects, stores and exposes real-time
    $\{r_i\}_i\subset V(G)$ robots' data;
    then sends instructions to the robots, e.g.,
    robots' movements.
    The Robot Middleware
    periodically collects
    the robots' Point of Access (PoA) attachment
    $\phi(r_i, R_i)\in\{0,1\}$,
    and a vector of sensor data
    $\sigma(r_i)~\in~\mathbb{R}^n$. 
    Using the aforementioned information,
    the Robot Middleware creates a contextual embedding~$\kappa(r_i)$
    \begin{align}
        \kappa \colon \{r_i\}_i &\to \mathbb{R}^n\\
        r_i &\mapsto \big(\phi(r_i,R_1),
        \dots, \phi(r_i,R_{N}), \sigma(r_i)\big) \notag
    \end{align}
    that is stored
    (via
    the Measurements API)
    in
    the Measurements building block,
    and exposed (via its own API) to the
    Plug-in layer (see Figure~\ref{fig:system}).
    Latter, a Plug-in uses the contextual
    embedding to elaborate real-time 
    navigation and PoA attachment 
    instructions $\phi(r_i,R_i)$, and forwards them to
    the Robot Middleware API.
    Finally, Robot Middleware
    sends the Plug-in instructions
    to the robots.
    \item \textbf{Network Control} building block collects, exposes and stores
    network and PoA context information.
    One of its main functionalities is to emulate
    network conditions.
    As well, it maps Virtual Functions (VF) and
    Virtual Links (VL) in the hardware graph,
    while storing and
    exposing the VF/VL mappings.
    The Network Control collects a vector with
    PoAs' context information $\iota(R_i)\in\mathbb{R}^m,~R_i\in V(G)$,
    so as the links' throughput
    $\lambda(n_1,n_2),~(n_1,n_2)\in E(G)$, and delay
    $d(n_1,n_2),~(n_1,n_2)\in E(G)$ between every
    robot, PoA, switch, and server
    in the hardware graph $G$.
    In addition, the Network Control exposes 
    the real-time PoA context information,
    links' delay, and throughput
    via its API; and stores
    the prior data
    in the Measurements building block using the Measurements API.
    To emulate network conditions, 
    Network Control retrieves
    $\lambda(\cdot)$ throughput, and
    $d(\cdot)$ delay  embeddings from
    the Measurements building block; and
    introduces artificial queuing
    delay
    $\psi(n_1,n_2)\ge0,~(n_1,n_2)\in E(G)$
    so as packet drop rate
    $\delta(n_1,n_2)\ge0$.
    As a result, the links
    $(n_1,n_2) \in E(G) $ in the hardware
    graph offer
    a delay of $\psi(n_1,n_2)+d(n_1,n_2)$, and
    a throughput of
    $\frac{1}{\delta(n_1,n_2)}\lambda(n_1,n_2)$.
    The Network Control API exposes
    operations to request both, queueing
    delay, and packet~drop.
    \vspace{0.5em} \\ %
    Additionally, the Network Control building block
    acts as a Virtual Infrastructure
    Manager (VIM)~\cite{mec-nfv} that maps VFs $\{v_i\}_i$ to hardware nodes
    $a(n)=\{v_1,\ldots,v_n\}, n\in V(G)$; and VLs in the hardware links, that is
    $a(n_1,n_2) = \{(v_1,v_2),\ldots, (v_{n-1},v_n)\}$.
    Both VFs, and VLs mappings are
    periodically stored and exposed by the
    Measurements component
    (using the Measurements API); and
    Plug-ins can issue new mappings
    over the exposed
    Network Control API.
    
    
    \item \textbf{Measurements} building block stores, and exposes an embedding history that is represented
    as a set 
    \begin{equation}
        \left\{ \{\kappa^t(r_i)\}_{r_i},
        \{a^t(n)\}_n,
        \{d^t(n_1,n_2)\}_{n_i},
        \{\lambda^t(n_1,n_2)\}_{n_i}
        \right\}_t
        \label{eq:historic}
    \end{equation}
    with $\kappa^t(r_i)$ denoting
    the contextual embedding of robot
    $r_i$ at time $t$. As shown in (\ref{eq:historic}), the
    embeddings history stores
    the VF/VL mappings,
    network delay, and throughput information.
    The embeddings history is exposed via
    the Measurements API
    to the Plug-in layer (see
    Figure~\ref{fig:system}).
\end{itemize}
\end{comment}
\begin{table}[!t]
    \centering
    \caption{Notation table }
    \begin{tabular}{|c||c|}
        \hline
        \textbf{Symbol} & \textbf{Definition} \\
        \hline
         $r_i$ & robot number $i\in\mathbb{N}$\\
        \hline
         $G$ & hardware graph\\
        \hline
         $V(G)$ & hardware graph nodes, e.g., a server \\
        \hline
          $E(G)$ & hardware graph edges, e.g., a wireless link\\
        \hline
          $\mathcal{S}$ & set of robotic services\\
        \hline  $S_i$ & a robotic service $S_i\in\mathcal{S}$\\
        \hline  $V(S_i)$ & set of VFs of robotic service $S_i$\\
        \hline $E(S_i)$ & set of VLs of robotic service $S_i$\\
        \hline  $D(S_i)$ & service $S_i$ latency requirement\\
       \hline   $R_i$ & Point of Access (PoA) number $i\in\mathbb{N}$\\
       \hline   $s_i$ & server number $i\in\mathbb{N}$\\
       \hline   $w_i$ & switch number $i\in\mathbb{N}$\\
       \hline   $\phi(r_i,R_i)$ & whether robot $r_i$ is attached to PoA $R_i$\\
       \hline   $\sigma(R_i)$ & signal strength
       \\
       \hline   $\kappa(r_i)$ & robot $r_i$ PoA attachment and sensor data\\
      \hline    $d(n_1,n_2)$ & delay between nodes $n_1,n_2\in V(G)$\\
      \hline    $\iota(R_i)$ & context information of PoA $R_i$\\
      \hline    $\lambda(n_1,n_2)$ & throughput in the link $(n_1,n_2)$\\
      \hline    $\psi(n_1,n_2)$ & artificial queuing delay in link $(n_1,n_2)$\\
     \hline     $\delta(n_1,n_2)$ & artifitial packet drop rate in link $(n_1,n_2)$\\
      \hline    $a(n)$ & set of VFs hosted at node $n$\\
      \hline    $a(n_1,n_2)$ & set of VLs hosted at link $(n_1,n_2)$\\ \hline
    \end{tabular}
    \label{tab:notation}
\end{table}





